On the density of zeros of linear combinations of Euler products for $\sigma>1$

It has been conjectured that the real parts of the zeros of a linear combination of two or more $L$-functions are dense in the interval $[1,\sigma^*]$, where $\sigma^*$ is the least upper bound of the real parts of such zeros. In this paper we show that this is not true in general. Moreover, we describe the optimal configuration of the zeros of linear combinations of orthogonal Euler products by showing that the real parts of such zeros are dense in subintervals of $[1,\sigma^*]$ whenever $\sigma^*>1$.

==> proof_main.tex <==

For easier reference, we state here a result often referred as Kronecker-Weyl's theorem (see Karatsuba and Voronin \cite[\S A.8]{karatsubavoronin}).
\begin{theorem}\label{theorem:kronecker}
Let be given a positive integer $n$ and a family $\Omega$ of continuous complex functions $H(\theta_1,\ldots,\theta_n)$ such that $H(\theta_1+m_1,\ldots,\theta_n+m_n)=H(\theta_1,\ldots,\theta_n)$ for every $(m_1,\ldots,m_n)\in\Z^n$ and every $(\theta_1,\ldots,\theta_n)\in[0,1]^n$. If $\Omega$ is uniformly bounded and equicontinuous, then for any $\lambda_1,\ldots,\lambda_n\in\R$ linearly independent over $\Q$ we have
\begin{equation}\label{eq:kronecker}
\lim_{T_2-T_1\rightarrow \infty}\frac{1}{T_2-T_1}\int_{T_1}^{T_2}H(\lambda_1 t,\cdots,\lambda_n t) dt = \int_{[0,1]^n} H(\theta_1,\ldots,\theta_n)d\theta_1\cdots d\theta_n
\end{equation}
uniformly with respect to $H\in\Omega$.\\
In particular we can take $(\lambda_1,\ldots,\lambda_n)=(\log p_1,\ldots, \log p_n)$, where $p_1,\ldots,p_n$ are distinct primes.
\end{theorem}

